Gaze-based Learning from Demonstration In Surgical Robotics

Surgical robotics is a rising field in medical technology and advanced robotics. Robot assisted surgery, or robotic surgery, allows surgeons to perform complicated surgical tasks with more precision, automation, and flexibility than is possible for traditional surgical approaches. The main type of robot assisted surgery is minimally invasive surgery, which could be automated and result in a faster healing time for the patient. The surgical robot we are particularly interested in is the da Vinci surgical system, which is developed and manufactured by Intuitive Surgical. In the current iteration of the system, the endoscopic camera arm on the da Vinci robot has to be manually controlled and calibrated by the surgeon during a surgical task, which interrupts the flow of the operation. The main goal of this capstone project is to automate the motion of the camera arm using a probabilistic model based on surgeon eye gaze data and da Vinci robot kinematic data.

==> PackagesLoadedbyTemplate.tex <==
% University of Pennsylvania Ph.D. Dissertation LaTeX Template packages

upennstyle.sty loads the following packages
\begin{itemize}
\item geometry 
\item fontenc
\item babel
\item csquotes
\item amsthm
\item amsmath
\item amssymb
\item amsfonts
\item amscd
\item calc
\item graphicx
\item float
\item caption
\item multirow
\item blindtext
\item verbatim
\item parskip
\item titlesec
\item appendix
\item setspace
\item array
\item tabularx
\item booktabs
\item pdflscape
\item hyperref
\item tocloft
\end{itemize}

sampledissertation.tex loads the following packages
\begin{itemize}
\item upennstyle
\item natbib
\end{itemize}
